Through the Haze: a Non-Convex Approach to Blind Gain Calibration for Linear Random Sensing Models

Computational sensing strategies often suffer from calibration errors in the physical implementation of their ideal sensing models. Such uncertainties are typically addressed by using multiple, accurately chosen training signals to recover the missing information on the sensing model, an approach that can be resource-consuming and cumbersome. Conversely, blind calibration does not employ any training signal, but corresponds to a bilinear inverse problem whose algorithmic solution is an open issue. We here address blind calibration as a non-convex problem for linear random sensing models, in which we aim to recover an unknown signal from its projections on sub-Gaussian random vectors, each subject to an unknown positive multiplicative factor (or gain). To solve this optimisation problem we resort to projected gradient descent starting from a suitable, carefully chosen initialisation point. An analysis of this algorithm allows us to show that it converges to the exact solution provided a sample complexity requirement is met, i.e., relating convergence to the amount of information collected during the sensing process. Interestingly, we show that this requirement grows linearly (up to log factors) in the number of unknowns of the problem. This sample complexity is found both in absence of prior information, as well as when subspace priors are available for both the signal and gains, allowing a further reduction of the number of observations required for our recovery guarantees to hold. Moreover, in the presence of noise we show how our descent algorithm yields a solution whose accuracy degrades gracefully with the amount of noise affecting the measurements. Finally, we present some numerical experiments in an imaging context, where our algorithm allows for a simple solution to blind calibration of the gains in a sensor array.

==> subspace_old.tex <==
\section{Blind Calibration with Subspace Priors}
		\label{sec:blind-calibration-with-subspace-priors}
		
			%			\begin{figure}[t]
			%				\centering
			%				\includegraphics[width=3in]{bcsubcoh.pdf}
			%				\caption{\label{fig:subscoh}Geometric intuition on the role of coherence in \eqref{eq:bcpk}: for $m = 3$, $h = 2$ we have highlighted $\cl G_\rho = \vone_m + \bs 1^\perp_m \cap \rho \bb B^m_\infty$ for $\rho = 0.99$, and $\cl B_\rho$ as the intersection of $\cl G_\rho$ with the subspace $\cl B$ (dashed: identity, dotted: DCT).}
			%			\end{figure}
			
			We now apply the same principles developed in Sec.~\ref{sec:nonconv} to define a simple modification of Alg.~\ref{alg1} specialised to the sensing model in Def.~\ref{def:modelsub}, \ie when $\y_l = \diag(\bs B \bs b) \A_l {\bs Z} {\bs z} \in \R^m$. Hereafter ${\bs x} \in \cl Z \subset \bb R^n$, ${\bs g} = \bs B \bs b \in \cl B \cap (\vone_m + \onep) \subset \bb R^m$, \ie we assume a subspace prior exists on the signal and the gains. Resuming our previous methodology of Sec.~\ref{sec:prelims}, we assume that the gains ${\bs g} = {\bs B} \bs b = \vone_m + \bs e$ but set ${\bs e} = \bs B^\perp \bs b^\perp  \in \onep \cap \rho \B^m_\infty$, where $\bs B^\perp$ spans $\onep$. To fix ideas, $\bs B^\perp$ could be constructed by taking $h-1$ basis elements of the discrete cosine transform (DCT) excluding the so-called DC component. Hence, we have that $\bs B \coloneqq \begin{bmatrix} \tfrac{\vone_m}{\sqrt{m}}  & \bs B^\perp \end{bmatrix}$, so for this model $\|{\bs g}\|_1 = m$ would fix the coefficients $\bs b \coloneqq \begin{bmatrix}\sqrt m & (\bs b^\perp)^\top\end{bmatrix}^\top$. Since we can always apply a scaling factor to the gains ${\bs g} \in \R^m_+$, this choice of $\bs b$ is still quite general. In this setup, the blind calibration problem is reduced to the following definition.
			
			\begin{definition}[Non-convex Blind Calibration Problem with Subspace Priors]
				Given two subspaces $\cl B \subset \bb R^m$ and $\cl Z \subset \bb R^n$, with dimension $h := \dim \cl B \leq m$ and $k := \dim \cl Z \leq n$, and with orthonormal bases $\bs B \in \R^{m\times h}$ and ${\bs Z} \in \R^{n \times k}$ (\ie tight frames), respectively, we define {\em non-convex blind calibration with subspace priors} the optimisation problem
					\begin{equation}%
					\label{eq:bcpk}
					(\bar{{\bs z}}, \bar{\bs b}) \coloneqq {\mathop{\argmin}_{({\bs \zeta},{\bs \beta}) \in {\cl Z} \times \cl B_\rho}} \tfrac{1}{2mp} {\ts \sum_{l=1}^{p} \left\Vert \diag({\bs B }{\bs \beta}) \A_l {\bs Z} {\bs \zeta} - \y_l\right\Vert^2_2},
					\end{equation}%
				where 
				\begin{equation}
				\label{eq:subconstr}
				{\cl B}_\rho \coloneqq \left\{\bs v = \begin{bsmallmatrix} \sqrt m \\ \bs v^\perp \end{bsmallmatrix}
				\in \R^h : \bs B \bs v \in \vone_m + \bs 1^\perp_m \cap \rho \bb B^m_\infty\right\},
				\end{equation}
				given $\y_l = \diag({\bs B}{\bs b}) \A_l {\bs Z} {\bs z} \in \R^m$, $l \in [p]$ as in Def.~\ref{def:modelsub}.
			\end{definition}
			Moreover, we also define\footnote{Hereafter $\mu_{\max}$ always refers to $\bs B$, as shall be clear from the context.} the \emph{coherence} of $\bs B$ as 
			\begin{equation}
				\label{eq:mumax}
				\ts\mu_{\max} := \sqrt\frac{m}{h} \max_{i \in [m]} \|\bs B^\top \bs c_i\|^2_2 \, \in \, [1, \sqrt\frac{m}{h}].    
			\end{equation}
	        This quantity appears in \cite{AhmedRechtRomberg2014} and has a fundamental role in characterising $\bs B$ and its effect on the possibility of recovering $\bs b$. It measures how evenly the energy of $\bs B$ is distributed among its rows, given that the basis vectors are orthonormal. In particular, two classical examples are in order. As mentioned above, we could form $\bs B$ as $h$ basis elements drawn at random from the $m$ that define the DCT on $\R^m$; this actually leads to a low-coherence $\bs B$ whose $\mu_{\max}$ is close to $1$. On the other hand, if
	        \footnote{This case is not possible in our model since $\tfrac{\vone_m}{\sqrt m}$ must be a basis vector; it is however easy to find highly coherent examples of $\bs B$ containing $\frac{\vone_m}{\sqrt{m}}$ and working on the remaining $h-1$ basis vectors of $\bs B^\perp$.} 
	        $\bs B \coloneqq \begin{bsmallmatrix}
	        \bs I_h \\ \vzer_{m-h \times h} \end{bsmallmatrix}$ it is straightforward that $\mu_{\max} = \sqrt\frac{m}{h}$, \ie the worst case setting in which only $h$ out of $m$ rows are contributing to the energy in $\bs B$. We shall use this quantity in deriving the sample complexity for the known subspace case. 

			Let us now proceed by taking the gradient of the objective function
			\begin{equation}
				f^{\rm s}({\bs \zeta},{\bs \beta}) \coloneqq  \tfrac{1}{2mp} {\ts \sum_{l=1}^{p} \left\Vert \diag({\bs B}{\bs \beta}) \A_l {\bs Z} {\bs \zeta} - \y_l\right\Vert^2_2},
			\end{equation}
			that is the vector $\bs\nabla f^{\rm s}({\bs \zeta},{\bs \beta}) \coloneqq 
			\begin{bsmallmatrix} \bs\nabla_{{\bs \zeta}} f^{\rm s}({\bs \zeta},{\bs \beta})^\top &  \bs\nabla_{{\bs \beta}} f^{\rm s}({\bs \zeta},{\bs \beta})^\top  \end{bsmallmatrix}^\top$. 
			Firstly, in the signal-domain subspace we have 
			\begin{align}
				\bs\nabla_{{\bs \zeta}} f^{\rm s}({\bs \zeta},{\bs \beta}) & =  \tfrac{1}{mp} \ts\sum^p_{l=1} {\bs Z}^\top \A^\top_l \diag({\bs B}{\bs \beta}) \left(\diag({\bs B}{\bs \beta}) \A_l {\bs Z} {\bs \zeta} - \diag({\bs B \bs b}) \A_l {\bs Z} {\bs z}\right) \nonumber \\ 
				& = \tfrac{1}{mp} \ts\sum_{i,l}  (\bs c^\top_i {\bs B}{\bs\beta}){\bs Z}^\top  \ail \left[(\bs c^\top_i {\bs B}{\bs\beta})  \ail^\top \bs Z \bs\zeta  - (\bs c^\top_i {\bs B}{\bs b}) \ail^\top \bs Z \bs z\right] \nonumber \\
				& = {\bs Z}^\top \bs\nabla_{\bxi} f(\bxi,{\bs \gamma})\big\vert_{\bxi = {\bs Z} {\bs \zeta}, {\bs \gamma} = {\bs B}{\bs \beta}}
				\label{eq:gradw}
			\end{align}
			Then we can take the partial derivatives for the components $\beta_j, j\in[h]$, yielding
			\begin{align*}
				\frac{\partial}{\partial \beta_j}  f^{\rm s}({\bs \zeta},{\bs \beta}) & \coloneqq \tfrac{1}{mp} \ts\sum^p_{l=1} \left(\frac{\partial}{\partial \beta_j} (\sum^{h}_{t=1} {\bs B}_{\cdot, t} \beta_t)\right)^\top \diag(\A_l {\bs Z} {\bs \zeta}) \left(\diag({\bs B}{\bs \beta}) \A_l {\bs Z} {\bs \zeta} - \diag({\bs B \bs b}) \A_l {\bs Z} {\bs z}\right) \\
				& = \tfrac{1}{mp} \ts\sum_{i,l} ({\bs B}^\top_{\cdot,j} {\bs c}_i)  ( \ail^\top {\bs Z} {\bs\zeta}) \left[({\bs c}^\top_i {\bs B}{\bs\beta}) \ail^\top \bs Z \bs\zeta  - ({\bs c}^\top_i {\bs B} {\bs b}) \ail^\top \bs Z \bs z\right] \\
				& = {\bs B}^\top_{\cdot,j} \bs\nabla_{{\bs \gamma}} f(\bxi,{\bs \gamma})\big\vert_{\bxi = {\bs Z} {\bs \zeta}, {\bs \gamma} = {\bs B}{\bs \beta}}.
			\end{align*}
			where $\bs B_{\cdot,j} \in \R^m, j\in[h]$ denotes the columns of $\bs B$; thus, we can collect 
			\begin{align}
				\label{eq:gradz}
				\bs\nabla_{{\bs \beta}} f^{\rm s}({\bs \zeta},{\bs \beta}) & = \tfrac{1}{mp} {\bs B}^\top \left(\ts\sum_{i,l} ( \ail^\top {\bs Z} {\bs\zeta}) \left[({\bs c}^\top_i {\bs B}{\bs\beta}) \ail^\top \bs Z \bs\zeta  - ({\bs c}^\top_i {\bs B} {\bs b}) \ail^\top \bs Z \bs z\right] {\bs c_i}\right) \nonumber \\
				& =  {\bs B}^\top \bs\nabla_{{\bs \gamma}} f(\bxi,{\bs \gamma})\big\vert_{\bxi = {\bs Z} {\bs \zeta}, {\bs \gamma} = {\bs B}{\bs \beta}}.
			\end{align}
			\mtodo{This part is {\em wrong} as it is. It should be rewritten with a definition of $\bs\nabla^\perp f^{\rm s}(\bs \zeta, \bs \beta)$, of $\bs\nabla^\perp_{\bs \beta} f(\bs\zeta,\bs\beta)$, etc.}
			\mtodo{Replace all instances of the gradient with the new explanation and definition.}
			Note that in the gain-domain subspace~\eqref{eq:subconstr} enforces $\beta_1 = \sqrt{m}$ and that ${ \langle {\bs B}_{\cdot,j}, {\bs c}^\perp_i \rangle } = { \langle {\bs B}_{\cdot,j}, {\bs c}_i \rangle }$ for $j > 1$ (because these columns are those of $\bs B^\perp$, which spans $\onep$). Thus, when the constraint is enforced it is legitimate to say that the variations on $\beta_1$ are always null (\ie the variations are again taken on $\onep$, or equivalently $\beta_1 \coloneqq \sqrt m$ at each step of the optimisation) and 
			\[
				\bs\nabla_{{\bs \beta}} f^{\rm s}({\bs \zeta},{\bs \beta}) = {\bs B}^\top \bs\nabla^\perp_{{\bs \gamma}} f(\bxi,{\bs \gamma})\big\vert_{\bxi = {\bs Z} {\bs \zeta}, {\bs \gamma} = {\bs B}{\bs \beta}} = \left.\begin{bsmallmatrix} 0 \\ ({\bs B^\perp})^\top \bs\nabla^\perp_{{\bs \gamma}} f(\bxi,{\bs \gamma}) \end{bsmallmatrix}\right\vert_{\bxi = {\bs Z} {\bs \zeta}, {\bs \gamma} = {\bs B}{\bs \beta}}.
			\]
			
			The definitions introduced in Sec.~\ref{sec:nonconv} also require minimal changes to be adapted to the sensing model with subspace priors. Indeed, we have just developed the gradient components of $\bs\nabla f^{\rm s} ({\bs \zeta},{\bs \beta})$, that can be obtained by those of $\bs\nabla^\perp f(\bxi,{\bs \gamma})$. Moreover, it is straightforward to obtain the initialisation ${\bs \zeta}_0$ in the signal-domain subspace from $\bxi_0$ as ${\bs \zeta}_0 \coloneqq {\bs Z}^\top \bxi_0$, while we can let ${\bs \beta}_ 0 \coloneqq \begin{bsmallmatrix} \sqrt m \\ \vzer_{h-1}\end{bsmallmatrix}$ equivalently to what we adopted in Sec.~\ref{sec:nonconv}. By our choice of ${\bs Z}$ and recalling $\x = {\bs Z} {\bs z}$ we see that the initialisation is still so that
			\[
				\Ex {\bs \zeta}_0 = \tfrac{1}{m p}  
				\ts\sum_{i,l} (\bs c^\top_i \bs B \bs b) \underbrace{\Ex {\bs Z}^\top \ail  \ail^\top {\bs Z}}_{\I_k} \bs z  = {\bs z} ,
			\]
			thus yielding an unbiased estimate of the exact signal-domain solution. The neighbourhood of the global minimiser\footnote{The $^\star$ notation is not required since, by the assumptions in this model, $\|{\bs g}\|_1 = m$. % consistently with the enforced ${\bs \gamma} = \vone_m + {\bs B}{\bs \beta} : {\bs B}{\bs \beta} \in \onep$.
			} $({\bs z},{\bs b})$ (for which we require at least $mp \geq k + h$) is then defined using the distance  
			\begin{equation}
				{\Delta}({\bs \zeta},{\bs \beta}) \coloneqq \|{\bs \zeta}-{\bs z}\|^2_2 + \tfrac{\|{\bs z}\|^2_2}{m}\|{\bs \beta}- {\bs b}\|^2_2
				\label{eq:dist_subs}
			\end{equation}
			and noting that $({\bs \zeta}-{\bs z})^\top ({\bs \zeta}-{\bs z}) \equiv (\bxi-\x)^\top (\bxi-\x),  ({\bs \beta}- {\bs b})^\top ({\bs \beta}- {\bs b})\equiv ({\bs \gamma}-{\bs g})^\top ({\bs \gamma}-{\bs g})$ with our choices of ${\bs B},{\bs Z}$ as tight frames. Indeed, this guarantees that~\eqref{eq:dist_subs} has the same value as~\eqref{eq:dist}, so we can modify Def.~\ref{def:neighbour} to express it in terms of the coefficients in their respective subspaces, \ie 
			\begin{equation}
				{{\cl D}^{\rm s}_{\kappa,\rho}} \coloneqq \{({\bs \zeta},{\bs \beta})\in \R^k \times {\cl B}_\rho : \Delta({\bs \zeta},{\bs \beta}) \leq \kappa^2 \|{\bs z}\|^2_2\}, \ \rho \in [0, 1).
			\end{equation}
			Thus, we are allowed to use the very same theory to obtain analogue results with respect to Prop.~\ref{prop:init} and~\ref{prop:regu}, anticipating the advantage a lower sample complexity given by the use of subspace priors. In fact, it is simply shown that the former propositions are special cases of Prop.~\ref{prop:initsub} and~\ref{prop:regusub}, as obtained when $\cl B \coloneqq \bb R^m$ and $\cl Z \coloneqq \bb R^n$, \ie $h=m$, $k=n$. Hence, to show convergence we will have to prove Prop.~\ref{prop:initsub} and~\ref{prop:regusub}.
			
			% ALGORITHM
			\begin{algorithm}[!t]
				{   \small
					\begin{algorithmic}[1]
						\STATE Initialise ${\bs \zeta}_0 \coloneqq \tfrac{1}{m p}
						\sum^{p}_{l = 1} \left(\A_l {\bs Z} \right)^\top \y_l,
						\, {\bs \beta}_0 \coloneqq \begin{bsmallmatrix}
						\sqrt m \\ \vzer_h
						\end{bsmallmatrix}, \, j \coloneqq0$. 
						\WHILE{stop criteria not met}
						% \item[] COMMENT{Line search w.r.t. $\bxi,{\bs \beta}$}
						\STATE $\begin{cases} 
						\mu_{\bs \zeta} \coloneqq \argmin_{\upsilon \in \R} f^{\rm s}({\bs \zeta}_{j}-\upsilon\bs\nabla_{\bs \zeta} f^{\rm s}({{\bs \zeta}_{j}, {\bs \beta}_ {j}}), {\bs \beta}_ {j}) \\
						\mu_{{\bs \beta}} \coloneqq \argmin_{\upsilon \in \R} f^{\rm s}({\bs \zeta}_{j},{\bs \beta}_ {j}-\upsilon\bs\nabla_{\bs \beta} f^{\rm s}({{\bs \zeta}_{j}, {\bs \beta}_ {j}})) 
						\end{cases}$
						\STATE ${\bs \zeta}_{j+1} \coloneqq {\bs \zeta}_{j} - \mu_{\bs \zeta} \bs\nabla_{\bs \zeta} f^{\rm s}({{\bs \zeta}_{j}, {\bs \beta}_ {j}})$
						\STATE $\check{{\bs \beta}}_{j+1} \coloneqq {\bs \beta}_ {j} - \mu_{\bs \beta} \, \bs\nabla_{\bs \beta} f^{\rm s}({{\bs \zeta}_{j}, {\bs \beta}_ {j}})$ % COMMENT{Update estimates}
						\STATE ${{\bs \beta}}_{j+1} \coloneqq{\cl P}_{\cl B_\rho} \check{{\bs \beta}}_{j+1}$
						\STATE $j \coloneqq j + 1$
						\ENDWHILE
					\end{algorithmic}
				}
				\caption{\label{alg2} Non-Convex Blind Calibration by Projected Gradient Descent with Known Signal and Gain Subspaces.}
			\end{algorithm}
			
			For what concerns the descent algorithm, a modification is straightforwardly obtained as Alg.~\ref{alg2}. The main difference is that the optimisation is carried out on the subspace coefficients $\bs \zeta$ and $\bs \beta$ rather than the signal and gains, with the gradient expressions given in~\eqref{eq:gradw} and~\eqref{eq:gradz}. The descent will run from $({\bs \zeta}_0, {\bs \beta}_ 0)$ up to $({\bs \zeta}_j, {\bs \beta}_ j)$ at the $j$-th iteration with the updates specified in steps 4:-6:. Again, the gradient update in the gain-domain subspace is followed by the projection on $\cl B_\rho$, which is a closed convex set. This is still algorithmically simple and not employed in the numerical results, as for $\cl G_\rho$ in absence of subspace priors. % ; this projection is simply ${\cl P}_{\cl B_\rho}({{\bs \beta}}) = {\bs B}^\top {\cl P}_{\rho \B^m_\infty} ({\bs B^\perp}{{\bs \beta}})$ for ${\bs \beta} \in \R^h$. % , which still satisfies the constraint that since by construction ${\bs B}^\top \vone_m=\vzer_h$. 
			
			It remains to be established how the main theoretical statements are modified. We now introduce an extension of our main results in Sec.~\ref{sec:recguars}. The proofs of the next statements are reported in App.~\ref{sec:appC} and rely on the fact that the technical arguments used in proving the results of Sec.~\ref{sec:recguars} are actually a special case of those in the subspace case, with a lower sample complexity due to the low-dimensional description of the signal and gains.  			
			
			Firstly, we have that the sample complexity requirements for the initialisation in Prop.~\ref{prop:init} are essentially reduced to $mp \gtrsim (k+h)\log n$.
			
			\begin{proposition}[Initialisation Proximity with Subspace Priors]
				\label{prop:initsub}
				Let $({\bs \zeta}_0,{\bs \beta}_ 0)$ be as in Alg.~\ref{alg2}. For any ${\delta} \in (0,1)$, $t \geq 1$, provided $\ts mp \gtrsim {\delta}^{-2} (k+h) \log \tfrac{n}{\delta} $ and  $n \gtrsim t \log mp $, with probability exceeding
				\begin{equation}
				\label{eq:bounds1}
				1 - C e^{- c {\delta}^2 m p} - (mp)^{-t}
				\end{equation}
				for some $C,c>0$, we have that $\|{\bs \zeta}_0 - {\bs z} \|_2 \leq {\delta} \|{\bs z}\|_2$. Thus, $({\bs \zeta}_0,{\bs \beta}_ 0) \in
				{\cl D}^{\rm s}_{{\kappa},\rho}$ with the same probability and $\kappa \coloneqq \sqrt{\delta^2+\rho^2}$.
			\end{proposition}
			
			The regularity condition in Prop.~\ref{prop:regu} is similarly obtained with reduced requirements on the amount of observations, \ie 
$mp \gtrsim \delta^{-2} (k + \mu^2_{\max} h)\, \log^2(m(p+n))\log(\frac{1}{\delta})$.

			\begin{proposition}[Regularity Condition with Subspace Priors]
				\label{prop:regusub}
				For any $\delta \in (0,1),\rho \in [0,1)$, $t \geq 1$, provided $\rho < \tfrac{1-4\delta}{31}$ and 
                % \new
                {\begin{align*}
                  \label{eq:glob-requirements-reg-prior}
                   \ts n&\ts \gtrsim t \log(mp),\\
                   \ts mp&\ts \gtrsim \delta^{-2} (k + \mu^2_{\max} h)\, \log^2(m(p+n))\log(\frac{1}{\delta}),            
                \end{align*}}
                with probability exceeding $1 - C (mp)^{-t}$ for some $C>0$, we have for all $({\bs \zeta},{\bs \beta}) \in {\cl D}^{\rm s}_{{\kappa},\rho}$,
				\begin{align}
					\left\langle \bs\nabla f^{\rm s}({\bs \zeta}, {\bs \beta}), \left[\begin{smallmatrix} {\bs \zeta}-{\bs z} \\ {\bs \beta}- {\bs b} \end{smallmatrix}\right] \right\rangle  \geq \tfrac{1}{2} \eta\, {\Delta}({\bs \zeta},{\bs \beta}) \\
					\|\bs\nabla f^{\rm s}({\bs \zeta}, {\bs \beta}) \|^2_2 \leq
					L^2\ {\Delta}({\bs \zeta},{\bs \beta}) 
				\end{align}
				where $\eta \coloneqq 2 (1-31\rho-4\delta)$, $L\coloneqq 8\sqrt{2}[1+(1+\kappa)\|\bs z\|_2]$. 
			\end{proposition}
			
            % \mtodo{Do we have to say this below since the proofs are established for the known subspace model first and then extended to full domain. The sentence below seems to say the converse even if it targets here the logical chaining of the steps.}
			% Since we have only generalised Prop.~\ref{prop:init} and Prop.~\ref{prop:regu} to the case of known subspaces addressed by Alg.~\ref{alg2}, convergence to the global minimiser is granted by the same steps that resulted in Thm.~\ref{theorem:convergence}. This follows from the fact we can seamlessly replace the initial assumptions of Thm.~\ref{theorem:convergence} since the relationship between the distances is preserved (again, due to the choice of tight frames $\bs Z, \bs B$ to model $(\x,{\bs g})$). The only change is indeed in the sample complexity required to achieve provable convergence.
			
			Given Prop.~\ref{prop:initsub} and~\ref{prop:regusub}, we finally obtain a more general version of Thm.~\ref{theorem:convergence} as follows.
			\begin{theorem}[Provable Convergence to the Exact Solution with Subspace Priors]
                          \label{theorem:convergence-subs}
                          Given $\delta \in (0,1), t\geq1$, provided $\rho < \tfrac{1-4\delta}{31}$ and  
$n \gtrsim t \log(mp)$, $mp \gtrsim \delta^{-2} (k + \mu^2_{\max} h)\, \log^2(m(p+n))\log(\frac{1}{\delta})$,            
                          with probability exceeding $1 - C (mp)^{-t}$ for some $C>0$, we have that Alg.~\ref{alg2} with $\mu_\bxi \coloneqq \mu$, $\mu_{\bs \gamma} \coloneqq \mu \tfrac{m}{\|\x^\star\|^2_2}$ has distance decay
                          \begin{equation}
                            {\Delta}({\bs \zeta}_j,{\bs \beta}_j) \leq
                            \big(1-\eta \mu + \tfrac{L^2}{\tau} \mu^2 \big)^j \big(\delta^2+\rho^2)\|\x^\star\|^2_2, \quad {(\bs \zeta_j, {\bs \beta}_j)\in {{\cl D}}^{\rm s}_{\kappa,\rho}}
                            \label{eq:convres}
                          \end{equation}
                          at any iteration $j > 0$  provided $\mu \in \big(0, \tfrac{\tau \eta}{L^2} \big)$, $\tau \coloneqq \min\{1,\tfrac{\|\x^\star\|^2_2}{{m}}\}$. Hence, ${\Delta}({\bs \zeta}_j,{\bs \beta}_j)\underset{j\rightarrow\infty}{\longrightarrow}0$.
			\end{theorem}
		
			Thus, subspace priors allow for a provably convergent application of Alg.~\ref{alg2}. Let us note that $mp \gtrsim \delta^{-2} (k + \mu^2_{\max} h)\, \log^2(m(p+n))\log(\frac{1}{\delta})$ is a clearly more stringent requirement than $mp \gtrsim (k+h) \log n$, emerging from Prop.~\ref{prop:initsub}. % This is due to the fact we have made no assumption on the subspace $\cl B$. % (\eg on the coherence of the frame $\bs B$)
			% Further assumptions on the tight frame $\bs B$, such as fixing its coherence, could in fact allow us to have a dependency on $k+h$ rather than $k+m$; we have however chosen to adopt a worst-case perspective that does not depend explicitly on the said coherence or on the structure of $\bs B$. % with a multiplicative factor depending 
\new{However, we see that if $\mu_{\max} \simeq 1$, and if $h$ and $k$ are small before $m$, having $p=1$ is allowed by the requirement; this will be also confirmed in our experiments, provided that both $k \ll n$, $h \ll m$ and $\mu_{\max}$ is sufficiently small. This allows for a single-snapshot application of our setup and algorithm to the blind calibration of sensors with side information regarding the subspaces to which $(\x,{\bs g})$ belong.} 
	
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "iai_blindcalibration_2016"
%%% End:

